Deep Functional Predictive Control for Strawberry Cluster Manipulation using Tactile Prediction

This paper introduces a novel approach to address the problem of Physical Robot Interaction (PRI) during robot pushing tasks. The approach uses a data-driven forward model based on tactile predictions to inform the controller about potential future movements of the object being pushed, such as a strawberry stem, using a robot tactile finger. The model is integrated into a Deep Functional Predictive Control (d-FPC) system to control the displacement of the stem on the tactile finger during pushes. Pushing an object with a robot finger along a desired trajectory in 3D is a highly nonlinear and complex physical robot interaction, especially when the object is not stably grasped. The proposed approach controls the stem movements on the tactile finger in a prediction horizon. The effectiveness of the proposed FPC is demonstrated in a series of tests involving a real robot pushing a strawberry in a cluster. The results indicate that the d-FPC controller can successfully control PRI in robotic manipulation tasks beyond the handling of strawberries. The proposed approach offers a promising direction for addressing the challenging PRI problem in robotic manipulation tasks. Future work will explore the generalisation of the approach to other objects and tasks.

==> [IROS23] Deep Functional Predictive Control/notations.tex <==
Notations adopted on this paper

Tactile frames in tactile prediction:               x

Robot actions in tactile prediction:                a

Robot actions output of the d-MPC:              \tilde{a}

Stem position:                                      s

Predicted stem location:                         \hat{s}

Centreline of the sensor (reference):            $s_ref$

Error: \hat{s} – $s_ref$:                        $e_t$       

Angular velocity around centreline:                a 

Proportional gain PD:                             $k_p$

Derivative gain PD:                               $k_d$

==> [IROS23] Deep Functional Predictive Control/parts/tables.tex <==
%%%
%

\begin{table*}[tb!]
        \centering
        \caption{\centering Control performance for the PD and d-FPC in pushing a single strawberry along a linear trajectory.}
        \label{tab:control}
        \begin{tabular}{|c||c|c|c|c|c|c|}
            \hline
            Model & \begin{tabular}{@{}c@{}} Contact \\ zone \end{tabular} & \begin{tabular}{@{}c@{}}Stem max\\ disp. \end{tabular} & \begin{tabular}{@{}c@{}}Stem slip\\ instances \end{tabular} & \begin{tabular}{@{}c@{}}Disp. \\ integral \end{tabular} & \begin{tabular}{@{}c@{}}Action \\ integral \end{tabular} & \begin{tabular}{@{}c@{}}Comp.\\ time (ms) \end{tabular} \\\hline
            \multirow{3}{*}{\begin{tabular}{@{}c@{}}Open-loop\end{tabular}} & 1 & 0.80 $\pm$ 0.2 & 31.23 $\pm$ 4.3 & 0.83 $\pm$ 0.1 & - & - \\
            & 2 & 1.35 $\pm$ 0.2 & 50.19 $\pm$ 5.7 & 0.91 $\pm$ 0.1 & - & - \\
            & 3 & 0.91 $\pm$ 0.1 & 39.83 $\pm$ 3.2 & 0.86 $\pm$ 0.2 & - & - \\
            \hline
            \multirow{3}{*}{\begin{tabular}{@{}c@{}} PD\end{tabular}} & 1 & 0.65 $\pm$ 0.1 & 27.2 $\pm$ 6.5  & 0.75 $\pm$ 0.1 & 2.93 $\pm$ 0.7 & 18.73 $\pm$ 2 \\
             & 2 & \textbf{0.36} $\pm$ 0.0 & 10.2 $\pm$ 2.4 & 0.48 $\pm$ 0.0 & 5.12 $\pm$ 3.8 & 20.30 $\pm$ 1 \\
            & 3 & 0.63 $\pm$ 0.1 & 24.2 $\pm$ 1.6 & 0.47 $\pm$ 0.1 & 9.73 $\pm$ 5.4 & 19.73 $\pm$ 1 \\
           \hline
           \multirow{3}{*}{\begin{tabular}{@{}c@{}} \textbf{d-FPC}\end{tabular}} & 1 & \textbf{0.20} $\pm$ 0.0 & \textbf{5.0} $\pm$ 1.2  & \textbf{0.12} $\pm$ 0.0 & 3.74 $\pm$ 0.8 & 60.49 $\pm$ 6 \\
             & 2 & 0.43 $\pm$ 0.0 & \textbf{7.2} $\pm$ 0.7 & \textbf{0.18} $\pm$ 0.0 & 4.27 $\pm$ 1.2 & 55.02 $\pm$ 2 \\
            & 3 & \textbf{0.25} $\pm$ 0.1 & \textbf{6.0} $\pm$ 0.6 & \textbf{0.09} $\pm$ 0.0 & 4.57 $\pm$ 2.4 & 58.54 $\pm$ 3 \\
           \hline
        \end{tabular}
    \end{table*}
%

%%%

\begin{table*}[tb!]
        \centering
        \caption{\centering Comparison of the controllers in linear and circular pushing trajectories (* integral is the integral of the * magnitude.).}
        \label{tab:trajectory}
        \begin{tabular}{|c||c|c|c|c|c|}
            \hline
            Model & \begin{tabular}{@{}c@{}} Robot \\ trajectory \end{tabular} & \begin{tabular}{@{}c@{}}Stem max\\ disp. \end{tabular} & \begin{tabular}{@{}c@{}}Stem slip\\ instances \end{tabular} & \begin{tabular}{@{}c@{}} Disp.\\ integral \end{tabular} & \begin{tabular}{@{}c@{}} Action\\ integral \end{tabular} \\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} Open-loop\end{tabular}} & Linear & 1.21 $\pm$ 0.18 & 44.38 $\pm$ 10.3  & 0.88 $\pm$ 0.4  & -\\
             & Circular & 1.35 $\pm$ 0.46 & 48.18 $\pm$ 5.2 & 1.02 $\pm$ 0.5 & -\\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} PD\end{tabular}} & Linear & 0.58 $\pm$ 0.21 & 25.53 $\pm$ 4.2  & 0.63 $\pm$ 0.1 & 5.39 $\pm$ 6.2 \\
             & Circular & 1.20 $\pm$ 0.01 & 17.6 $\pm$ 2.0 & 0.44 $\pm$ 0.0 & 9.89 $\pm$ 0.8\\
           \hline
           \multirow{2}{*}{\begin{tabular}{@{}c@{}} \textbf{d-FPC}\end{tabular}} & Linear & \textbf{0.29} $\pm$ 0.04 & \textbf{8.11} $\pm$ 1.4  & \textbf{0.13} $\pm$ 0.0 &  4.49 $\pm$ 2.5\\
             & Circular & \textbf{0.54} $\pm$ 0.05 & \textbf{5.0} $\pm$ 1.5 & \textbf{0.22} $\pm$ 0.0 & 6.66 $\pm$ 0.8\\
           \hline
        \end{tabular}
    \end{table*}
%
%%%

%%%
\begin{table*}[tb!]
        \centering
        \caption{\centering Controller and open loop performances for Pushing a cluster of strawberries.}
        \label{tab:cluster}
        \begin{tabular}{|c||c|c|c|c|}
            \hline
            Model & \begin{tabular}{@{}c@{}} Robot \\ trajectory \end{tabular} & \begin{tabular}{@{}c@{}}Stem max\\ disp. \end{tabular} & \begin{tabular}{@{}c@{}}Stem slip\\ instances \end{tabular} & \begin{tabular}{@{}c@{}} Disp.\\ integral \end{tabular} \\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} Open-loop\end{tabular}} & Linear & 1.43 $\pm$ 0.30 & 49.33 $\pm$ 15.64  & 1.39 $\pm$ 0.33 \\
             & Circular & 1.29 $\pm$ 0.67 & 47.98 $\pm$ 6.33 & 1.19 $\pm$ 0.23 \\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} PD\end{tabular}} & Linear & 0.79 $\pm$ 0.21 & 29.4 $\pm$ 6.52  & 0.66 $\pm$ 0.21  \\
             & Circular & 1.14 $\pm$ 0.23 & 20.5 $\pm$ 2.69 & 0.56 $\pm$ 0.84 \\
           \hline
           \multirow{2}{*}{\begin{tabular}{@{}c@{}} \textbf{d-FPC}\end{tabular}} & Linear & \textbf{0.31} $\pm$ 0.08 & \textbf{17.1} $\pm$ 2.39  & 0.25 $\pm$ 0.03\\
             & Circular & \textbf{0.61} $\pm$ 0.11 & \textbf{9.5} $\pm$ 4.58 & 0.27 $\pm$ 0.18 \\
           \hline
        \end{tabular}
    \end{table*}
%

==> [IROS23]Video and Tactile Prediction_ for strawberry cluster manipulation/parts/tables.tex <==
%%%
%

\begin{table*}[tb!]
        \centering
        \caption{\centering Control performance for the PD and d-FPC in pushing a single strawberry along a linear trajectory.}
        \label{tab:control}
        \begin{tabular}{|c||c|c|c|c|c|c|}
            \hline
            Model & \begin{tabular}{@{}c@{}} Contact \\ zone \end{tabular} & \begin{tabular}{@{}c@{}}Stem max\\ disp. \end{tabular} & \begin{tabular}{@{}c@{}}Stem slip\\ instances \end{tabular} & \begin{tabular}{@{}c@{}}Disp. \\ integral \end{tabular} & \begin{tabular}{@{}c@{}}Action \\ integral \end{tabular} & \begin{tabular}{@{}c@{}}Comp.\\ time (ms) \end{tabular} \\\hline
            \multirow{3}{*}{\begin{tabular}{@{}c@{}}Open-loop\end{tabular}} & 1 & 0.80 $\pm$ 0.2 & 31.23 $\pm$ 4.3 & 0.83 $\pm$ 0.1 & - & - \\
            & 2 & 1.35 $\pm$ 0.2 & 50.19 $\pm$ 5.7 & 0.91 $\pm$ 0.1 & - & - \\
            & 3 & 0.91 $\pm$ 0.1 & 39.83 $\pm$ 3.2 & 0.86 $\pm$ 0.2 & - & - \\
            \hline
            \multirow{3}{*}{\begin{tabular}{@{}c@{}} PD\end{tabular}} & 1 & 0.65 $\pm$ 0.1 & 27.2 $\pm$ 6.5  & 0.75 $\pm$ 0.1 & 2.93 $\pm$ 0.7 & 18.73 $\pm$ 2 \\
             & 2 & \textbf{0.36} $\pm$ 0.0 & 10.2 $\pm$ 2.4 & 0.48 $\pm$ 0.0 & 5.12 $\pm$ 3.8 & 20.30 $\pm$ 1 \\
            & 3 & 0.63 $\pm$ 0.1 & 24.2 $\pm$ 1.6 & 0.47 $\pm$ 0.1 & 9.73 $\pm$ 5.4 & 19.73 $\pm$ 1 \\
           \hline
           \multirow{3}{*}{\begin{tabular}{@{}c@{}} \textbf{d-FPC}\end{tabular}} & 1 & \textbf{0.20} $\pm$ 0.0 & \textbf{5.0} $\pm$ 1.2  & \textbf{0.12} $\pm$ 0.0 & 3.74 $\pm$ 0.8 & 60.49 $\pm$ 6 \\
             & 2 & 0.43 $\pm$ 0.0 & \textbf{7.2} $\pm$ 0.7 & \textbf{0.18} $\pm$ 0.0 & 4.27 $\pm$ 1.2 & 55.02 $\pm$ 2 \\
            & 3 & \textbf{0.25} $\pm$ 0.1 & \textbf{6.0} $\pm$ 0.6 & \textbf{0.09} $\pm$ 0.0 & 4.57 $\pm$ 2.4 & 58.54 $\pm$ 3 \\
           \hline
        \end{tabular}
    \end{table*}
%

%%%

\begin{table*}[tb!]
        \centering
        \caption{\centering Comparison of the controllers in linear and circular pushing trajectories (* integral is the integral of the * magnitude.).}
        \label{tab:trajectory}
        \begin{tabular}{|c||c|c|c|c|c|}
            \hline
            Model & \begin{tabular}{@{}c@{}} Robot \\ trajectory \end{tabular} & \begin{tabular}{@{}c@{}}Stem max\\ disp. \end{tabular} & \begin{tabular}{@{}c@{}}Stem slip\\ instances \end{tabular} & \begin{tabular}{@{}c@{}} Disp.\\ integral \end{tabular} & \begin{tabular}{@{}c@{}} Action\\ integral \end{tabular} \\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} Open-loop\end{tabular}} & Linear & 1.21 $\pm$ 0.18 & 44.38 $\pm$ 10.3  & 0.88 $\pm$ 0.4  & -\\
             & Circular & 1.35 $\pm$ 0.46 & 48.18 $\pm$ 5.2 & 1.02 $\pm$ 0.5 & -\\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} PD\end{tabular}} & Linear & 0.58 $\pm$ 0.21 & 25.53 $\pm$ 4.2  & 0.63 $\pm$ 0.1 & 5.39 $\pm$ 6.2 \\
             & Circular & 1.20 $\pm$ 0.01 & 17.6 $\pm$ 2.0 & 0.44 $\pm$ 0.0 & 9.89 $\pm$ 0.8\\
           \hline
           \multirow{2}{*}{\begin{tabular}{@{}c@{}} \textbf{d-FPC}\end{tabular}} & Linear & \textbf{0.29} $\pm$ 0.04 & \textbf{8.11} $\pm$ 1.4  & \textbf{0.13} $\pm$ 0.0 &  4.49 $\pm$ 2.5\\
             & Circular & \textbf{0.54} $\pm$ 0.05 & \textbf{5.0} $\pm$ 1.5 & \textbf{0.22} $\pm$ 0.0 & 6.66 $\pm$ 0.8\\
           \hline
        \end{tabular}
    \end{table*}
%
%%%

%%%
\begin{table*}[tb!]
        \centering
        \caption{\centering Controller and open loop performances for Pushing a cluster of strawberries.}
        \label{tab:cluster}
        \begin{tabular}{|c||c|c|c|c|}
            \hline
            Model & \begin{tabular}{@{}c@{}} Robot \\ trajectory \end{tabular} & \begin{tabular}{@{}c@{}}Stem max\\ disp. \end{tabular} & \begin{tabular}{@{}c@{}}Stem slip\\ instances \end{tabular} & \begin{tabular}{@{}c@{}} Disp.\\ integral \end{tabular} \\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} Open-loop\end{tabular}} & Linear & 1.43 $\pm$ 0.30 & 49.33 $\pm$ 15.64  & 1.39 $\pm$ 0.33 \\
             & Circular & 1.29 $\pm$ 0.67 & 47.98 $\pm$ 6.33 & 1.19 $\pm$ 0.23 \\
            \hline
            \multirow{2}{*}{\begin{tabular}{@{}c@{}} PD\end{tabular}} & Linear & 0.79 $\pm$ 0.21 & 29.4 $\pm$ 6.52  & 0.66 $\pm$ 0.21  \\
             & Circular & 1.14 $\pm$ 0.23 & 20.5 $\pm$ 2.69 & 0.56 $\pm$ 0.84 \\
           \hline
           \multirow{2}{*}{\begin{tabular}{@{}c@{}} \textbf{d-FPC}\end{tabular}} & Linear & \textbf{0.31} $\pm$ 0.08 & \textbf{17.1} $\pm$ 2.39  & 0.25 $\pm$ 0.03\\
             & Circular & \textbf{0.61} $\pm$ 0.11 & \textbf{9.5} $\pm$ 4.58 & 0.27 $\pm$ 0.18 \\
           \hline
        \end{tabular}
    \end{table*}
%

==> notations.tex <==
Notations adopted on this paper

Tactile frames in tactile prediction:               x

Robot actions in tactile prediction:                a

Robot actions output of the d-MPC:              \tilde{a}

Stem position:                                      s

Predicted stem location:                         \hat{s}

Centreline of the sensor (reference):            $s_ref$

Error: \hat{s} – $s_ref$:                        $e_t$       

Angular velocity around centreline:                a 

Proportional gain PD:                             $k_p$

Derivative gain PD:                               $k_d$
